Clustering the Orion B giant molecular cloud based on its molecular emission

Previous attempts at segmenting molecular line maps of molecular clouds have focused on using position-position-velocity data cubes of a single line to separate the spatial components of the cloud. In contrast, wide field spectral imaging with large spectral bandwidth in the (sub)mm domain now allows to combine multiple molecular tracers to understand the different physical and chemical phases that constitute giant molecular clouds. We aim at using multiple tracers (sensitive to different physical processes) to segment a molecular cloud into physically/chemically similar regions (rather than spatially connected components). We use a machine learning clustering method (the Meanshift algorithm) to cluster pixels with similar molecular emission, ignoring spatial information. Simple radiative transfer models are used to interpret the astrophysical information uncovered by the clustering. A clustering analysis based only on the J=1-0 lines of 12CO, 13CO and C18O reveals distinct density/column density regimes (nH~100, 500, and >1000 cm-3), closely related to the usual definitions of diffuse, translucent and high-column-density regions. Adding two UV-sensitive tracers, the (1-0) lines of HCO+ and CN, allows us to distinguish two clearly distinct chemical regimes, characteristic of UV-illuminated and UV-shielded gas. The UV-illuminated regime shows overbright HCO+ and CN emission, which we relate to photochemical enrichment. We also find a tail of high CN/HCO+ intensity ratio in UV-illuminated regions. Finer distinctions in density classes (nH~7E3, and 4E4 cm-3) for the densest regions are also identified, likely related to the higher critical density of the CN and HCO+ (1-0) lines. The association of simultaneous multi-line, wide-field mapping and powerful machine learning methods such as the Meanshift algorithm reveals how to decode the complex information available in molecular tracers.

==> tex/tab_clusters.tex <==
Cluster nb. &  Area fraction  & $^{12}$CO & $^{13}$CO & HCO$^+$ & HCN & CS & C$^{18}$O & HNC & CN & SO & CCH & CH$_3$OH & N$_2$H$^+$       \\ 
\hline
0 & 51.5\% (72636 pixels) & 92.5\% & 61.5\% & 30.9\% & 14.6\% & 4.1\% & 2.2\% & 4.6\% & 3.3\% & 1.9\% & 6.8\% & 2.2\% & 1.2\% \\
1 & 29.3\% (41275 pixels) & 100.0\% & 100.0\% & 95.6\% & 76.9\% & 56.1\% & 56.7\% & 39.6\% & 37.7\% & 27.7\% & 25.0\% & 3.2\% & 1.7\% \\
2 & 7.9\% (11148 pixels) & 100.0\% & 100.0\% & 99.9\% & 95.1\% & 92.4\% & 99.9\% & 66.1\% & 56.5\% & 65.7\% & 22.9\% & 11.9\% & 8.2\% \\
3 & 4.3\% (6019 pixels) & 100.0\% & 100.0\% & 72.3\% & 33.2\% & 8.7\% & 10.4\% & 6.8\% & 3.6\% & 4.1\% & 5.3\% & 0.0\% & 0.8\% \\
4 & 2.2\% (3087 pixels) & 100.0\% & 100.0\% & 100.0\% & 99.9\% & 100.0\% & 96.5\% & 99.9\% & 99.8\% & 99.4\% & 97.5\% & 31.8\% & 18.9\% \\
5 & 1.5\% (2109 pixels) & 100.0\% & 100.0\% & 100.0\% & 99.2\% & 90.7\% & 53.0\% & 93.0\% & 93.7\% & 71.2\% & 93.4\% & 14.0\% & 8.2\% \\
6 & 1.1\% (1522 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 96.4\% & 94.3\% & 97.0\% & 45.6\% & 25.6\% & 20.5\% \\
7 & 0.6\% (866 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 52.7\% & 45.7\% \\
8 & 0.5\% (700 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 98.1\% & 100.0\% \\
9 & 0.4\% (620 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 97.9\% & 97.6\% & 96.9\% & 71.0\% & 16.3\% & 6.1\% \\
10 & 0.3\% (481 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 99.6\% & 100.0\% & 84.4\% & 71.1\% & 10.8\% \\
11 & 0.2\% (300 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 98.7\% & 87.7\% & 100.0\% & 10.3\% & 33.3\% & 0.7\% \\
12 & 0.2\% (284 pixels) & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 100.0\% & 99.6\% & 100.0\% & 95.8\% & 14.4\% & 4.9\% \\



==> tex/tab_clusters2.tex <==
Cluster nb. &  Area fraction  & $^{12}$CO & $^{13}$CO & HCO$^+$ & HCN & CS & C$^{18}$O & HNC & CN & SO & CCH & CH$_3$OH & N$_2$H$^+$       \\ 
\hline
0 & 21.6\% (30484 pixels) & 91.0\% & 47.2\% & 18.0\% & 8.3\% & 2.3\% & 1.4\% & 2.7\% & 1.3\% & 1.4\% & 5.3\% & 2.0\% & 1.1\% \\
1 & 12.0\% (16956 pixels) & 84.2\% & 30.4\% & 8.8\% & 5.0\% & 0.8\% & 0.0\% & 1.2\% & 0.8\% & 0.6\% & 2.1\% & 1.8\% & 1.1\% \\
2 & 3.5\% (4943 pixels) & 100.0\% & 98.9\% & 54.5\% & 27.6\% & 6.8\% & 1.2\% & 8.7\% & 5.5\% & 3.2\% & 15.9\% & 2.2\% & 1.4\% \\
3 & 10.2\% (14352 pixels) & 100.0\% & 100.0\% & 63.8\% & 34.1\% & 11.1\% & 2.9\% & 13.1\% & 10.5\% & 5.5\% & 14.4\% & 2.2\% & 1.3\% \\
4 & 9.5\% (13336 pixels) & 100.0\% & 100.0\% & 76.0\% & 41.9\% & 19.0\% & 11.6\% & 16.8\% & 14.1\% & 9.3\% & 13.6\% & 2.6\% & 1.1\% \\
5 & 10.0\% (14109 pixels) & 100.0\% & 100.0\% & 88.2\% & 58.7\% & 31.4\% & 26.4\% & 22.1\% & 20.1\% & 13.9\% & 16.9\% & 2.4\% & 1.2\% \\
6 & 17.6\% (24769 pixels) & 100.0\% & 100.0\% & 96.4\% & 81.6\% & 64.6\% & 70.0\% & 44.9\% & 42.8\% & 32.5\% & 27.3\% & 3.6\% & 1.8\% \\
7 & 11.1\% (15625 pixels) & 100.0\% & 100.0\% & 99.8\% & 94.3\% & 94.5\% & 100.0\% & 74.6\% & 66.2\% & 75.6\% & 41.7\% & 25.9\% & 19.0\% \\
8 & 4.6\% (6476 pixels) & 100.0\% & 100.0\% & 100.0\% & 99.9\% & 96.9\% & 99.8\% & 88.7\% & 95.1\% & 78.9\% & 65.7\% & 10.6\% & 4.2\% \\



==> tex/tab_clusters_contributions.tex <==
Cluster nb. & $^{12}$CO & $^{13}$CO & HCO$^+$ & HCN & CS & C$^{18}$O & HNC & CN & SO & CCH & CH$_3$OH & N$_2$H$^+$       \\ 
\hline
0 & 17.1\% & 9.2\% & 17.2\% & 11.9\% & 5.7\% & 3.8\% & 9.7\% & 10.5\% & 5.4\% & 20.6\% & 25.1\% & -6.9\% \\
1 & 49.5\% & 43.6\% & 41.7\% & 43.4\% & 31.2\% & 31.2\% & 36.8\% & 44.1\% & 30.2\% & 39.9\% & 13.4\% & 16.5\% \\
2 & 15.0\% & 21.9\% & 14.1\% & 13.9\% & 17.8\% & 28.8\% & 15.0\% & 12.6\% & 15.0\% & 9.3\% & 25.9\% & 22.0\% \\
3 & 4.5\% & 2.9\% & 2.7\% & 2.2\% & 1.4\% & 1.6\% & 1.7\% & 2.1\% & 1.8\% & 2.6\% & -20.6\% & -5.4\% \\
4 & 4.1\% & 6.1\% & 6.9\% & 8.2\% & 11.2\% & 9.0\% & 10.6\% & 8.4\% & 18.0\% & 8.7\% & 13.7\% & 12.7\% \\
5 & 1.7\% & 1.4\% & 3.3\% & 3.8\% & 3.8\% & 1.8\% & 4.0\% & 3.9\% & 4.7\% & 4.7\% & 2.7\% & 1.9\% \\
6 & 2.0\% & 3.1\% & 3.1\% & 2.9\% & 4.3\% & 4.2\% & 4.0\% & 2.6\% & 5.3\% & 1.7\% & 5.9\% & 6.6\% \\
7 & 1.8\% & 4.2\% & 4.5\% & 7.5\% & 13.4\% & 6.2\% & 8.9\% & 9.5\% & 8.0\% & 8.0\% & 14.3\% & 22.4\% \\
8 & 1.4\% & 2.9\% & 3.1\% & 2.6\% & 5.9\% & 6.7\% & 5.5\% & 2.8\% & 5.7\% & 2.3\% & 11.5\% & 27.8\% \\
9 & 1.2\% & 1.9\% & 1.5\% & 1.4\% & 1.7\% & 2.5\% & 1.2\% & 1.3\% & 1.4\% & 0.8\% & 2.0\% & 0.5\% \\
10 & 0.8\% & 1.5\% & 1.1\% & 1.1\% & 2.1\% & 2.6\% & 1.4\% & 1.0\% & 2.5\% & 0.7\% & 3.9\% & 1.2\% \\
11 & 0.4\% & 0.6\% & 0.4\% & 0.4\% & 0.7\% & 0.8\% & 0.5\% & 0.4\% & 1.1\% & 0.2\% & 1.4\% & 0.1\% \\
12 & 0.5\% & 0.7\% & 0.5\% & 0.6\% & 0.8\% & 0.7\% & 0.7\% & 0.6\% & 1.0\% & 0.6\% & 0.8\% & 0.5\% \\



==> tex/tab_clusters_mean_intensities.tex <==
Cluster nb. & $^{12}$CO             & $^{13}$CO & HCO$^+$ & HCN & CS & C$^{18}$O & HNC & CN & SO & CCH & CH$_3$OH & N$_2$H$^+$       \\ 
                  & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s & K$\cdot$km/s \\
\hline
0 & $12.1\pm13.7$ & $1.2\pm1.9$ & $0.4\pm0.5$ & $0.2\pm0.3$ & $0.04\pm0.15$ & $0.03\pm0.16$ & $0.06\pm0.19$ & $0.08\pm0.27$ & $0.02\pm0.14$ & $0.12\pm0.28$ & $0.01\pm0.15$ & $-0.00\pm0.19$ \\
1 & $61.6\pm18.6$ & $9.9\pm4.8$ & $1.5\pm1.0$ & $1.0\pm0.7$ & $0.41\pm0.36$ & $0.48\pm0.41$ & $0.41\pm0.36$ & $0.57\pm0.53$ & $0.22\pm0.21$ & $0.40\pm0.37$ & $0.01\pm0.15$ & $0.02\pm0.18$ \\
2 & $69.1\pm13.6$ & $18.4\pm4.3$ & $1.9\pm0.8$ & $1.1\pm0.5$ & $0.87\pm0.56$ & $1.64\pm0.90$ & $0.63\pm0.56$ & $0.60\pm0.33$ & $0.40\pm0.25$ & $0.35\pm0.27$ & $0.09\pm0.13$ & $0.09\pm0.33$ \\
3 & $38.4\pm6.9$ & $4.6\pm1.8$ & $0.7\pm0.3$ & $0.3\pm0.3$ & $0.13\pm0.16$ & $0.17\pm0.21$ & $0.13\pm0.18$ & $0.19\pm0.25$ & $0.09\pm0.16$ & $0.18\pm0.23$ & $-0.14\pm0.12$ & $-0.04\pm0.19$ \\
4 & $68.0\pm15.2$ & $18.5\pm9.7$ & $3.4\pm1.2$ & $2.4\pm0.8$ & $1.98\pm1.22$ & $1.85\pm1.60$ & $1.59\pm0.83$ & $1.45\pm0.48$ & $1.73\pm1.22$ & $1.17\pm0.41$ & $0.18\pm0.23$ & $0.18\pm0.41$ \\
5 & $42.5\pm12.0$ & $6.3\pm3.4$ & $2.3\pm0.7$ & $1.6\pm0.7$ & $0.98\pm0.93$ & $0.54\pm0.72$ & $0.88\pm0.50$ & $0.99\pm0.36$ & $0.66\pm0.71$ & $0.94\pm0.31$ & $0.05\pm0.14$ & $0.04\pm0.16$ \\
6 & $66.3\pm12.8$ & $18.7\pm4.8$ & $3.1\pm1.4$ & $1.8\pm0.6$ & $1.56\pm0.81$ & $1.75\pm0.91$ & $1.23\pm0.95$ & $0.91\pm0.31$ & $1.04\pm0.68$ & $0.46\pm0.28$ & $0.16\pm0.21$ & $0.19\pm0.36$ \\
7 & $108.1\pm10.3$ & $45.1\pm16.8$ & $7.8\pm2.9$ & $7.9\pm4.4$ & $8.51\pm8.22$ & $4.54\pm3.06$ & $4.75\pm3.02$ & $5.87\pm2.60$ & $2.74\pm2.63$ & $3.87\pm2.49$ & $0.66\pm0.89$ & $1.12\pm2.28$ \\
8 & $99.3\pm15.4$ & $38.9\pm5.8$ & $6.7\pm2.7$ & $3.4\pm1.3$ & $4.63\pm2.08$ & $6.06\pm1.08$ & $3.67\pm1.05$ & $2.15\pm0.73$ & $2.39\pm1.06$ & $1.39\pm0.70$ & $0.66\pm0.38$ & $1.73\pm0.84$ \\
9 & $100.5\pm12.5$ & $28.3\pm3.6$ & $3.6\pm1.2$ & $2.1\pm0.5$ & $1.52\pm0.42$ & $2.56\pm0.55$ & $0.91\pm0.30$ & $1.12\pm0.34$ & $0.65\pm0.25$ & $0.55\pm0.26$ & $0.13\pm0.11$ & $0.04\pm0.17$ \\
10 & $89.2\pm13.8$ & $28.7\pm3.1$ & $3.5\pm0.7$ & $2.1\pm0.5$ & $2.40\pm0.36$ & $3.48\pm0.74$ & $1.32\pm0.27$ & $1.13\pm0.25$ & $1.51\pm0.41$ & $0.63\pm0.20$ & $0.33\pm0.18$ & $0.11\pm0.15$ \\
11 & $59.9\pm6.2$ & $18.0\pm2.2$ & $2.2\pm0.4$ & $1.3\pm0.3$ & $1.20\pm0.37$ & $1.79\pm0.36$ & $0.76\pm0.24$ & $0.65\pm0.19$ & $1.05\pm0.40$ & $0.24\pm0.14$ & $0.18\pm0.12$ & $0.01\pm0.11$ \\
12 & $94.7\pm5.6$ & $23.0\pm3.1$ & $2.5\pm0.4$ & $2.1\pm0.4$ & $1.61\pm0.51$ & $1.53\pm0.42$ & $1.10\pm0.19$ & $1.18\pm0.19$ & $1.03\pm0.28$ & $0.82\pm0.18$ & $0.11\pm0.11$ & $0.08\pm0.13$ \\
\hline
total & $36.4\pm30.3$ & $6.6\pm8.2$ & $1.1\pm1.3$ & $0.6\pm1.0$ & $0.39\pm1.12$ & $0.45\pm0.92$ & $0.33\pm0.67$ & $0.38\pm0.70$ & $0.21\pm0.53$ & $0.30\pm0.52$ & $0.03\pm0.19$ & $0.03\pm0.32$ \\


==> tex/tab_masses_densities.tex <==
Quantity & (unit) & \multicolumn{13}{c}{Cluster nb.} \\
 & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &10 & 11 & 12 \\
\hline
$M_{\mathrm{CO}}$ & $(M_{\odot})$ & $1.17\times 10^{3}$ & $3.39\times 10^{3}$ & $1.03\times 10^{3}$ & $3.08\times 10^{2}$ & $2.80\times 10^{2}$ & $1.19\times 10^{2}$ & $1.34\times 10^{2}$ & $1.25\times 10^{2}$ & $9.26\times 10^{1}$ & $8.30\times 10^{1}$ & $5.71\times 10^{1}$ & $2.40\times 10^{1}$ & $3.58\times 10^{1}$ \\
$M_{\mathrm{dust}}$ & $(M_{\odot})$ & $8.94\times 10^{2}$ & $1.41\times 10^{3}$ & $6.28\times 10^{2}$ & $1.21\times 10^{2}$ & $2.50\times 10^{2}$ & $8.27\times 10^{1}$ & $1.10\times 10^{2}$ & $1.89\times 10^{2}$ & $1.87\times 10^{2}$ & $4.56\times 10^{1}$ & $4.72\times 10^{1}$ & $1.63\times 10^{1}$ & $1.91\times 10^{1}$ \\
$M_{\mathrm{CO}}/M_{\mathrm{dust}}$ & - & $1.31$ & $2.40$ & $1.63$ & $2.55$ & $1.12$ & $1.44$ & $1.22$ & $0.659$ & $0.496$ & $1.82$ & $1.21$ & $1.47$ & $1.87$ \\
$S$ & $(\mathrm{pc}^{2})$ & $2.22\times 10^{1}$ & $1.26\times 10^{1}$ & $3.41\times 10^{0}$ & $1.84\times 10^{0}$ & $9.45\times 10^{-1}$ & $6.46\times 10^{-1}$ & $4.66\times 10^{-1}$ & $2.65\times 10^{-1}$ & $2.14\times 10^{-1}$ & $1.90\times 10^{-1}$ & $1.47\times 10^{-1}$ & $9.19\times 10^{-2}$ & $8.70\times 10^{-2}$ \\
$V$ & $(\mathrm{pc}^{3})$ & $1.97\times 10^{2}$ & $6.63\times 10^{1}$ & $6.31\times 10^{0}$ & $1.19\times 10^{1}$ & $9.19\times 10^{-1}$ & $1.09\times 10^{0}$ & $3.18\times 10^{-1}$ & $1.37\times 10^{-1}$ & $9.93\times 10^{-2}$ & $8.27\times 10^{-2}$ & $5.65\times 10^{-2}$ & $2.78\times 10^{-2}$ & $2.57\times 10^{-2}$ \\
$n_{\mathrm{H}}^{\mathrm{CO}}$ & $(\mathrm{cm}^{-3})$ & $1.77\times 10^{2}$ & $1.52\times 10^{3}$ & $4.84\times 10^{3}$ & $7.71\times 10^{2}$ & $9.05\times 10^{3}$ & $3.26\times 10^{3}$ & $1.26\times 10^{4}$ & $2.72\times 10^{4}$ & $2.78\times 10^{4}$ & $2.98\times 10^{4}$ & $3.01\times 10^{4}$ & $2.56\times 10^{4}$ & $4.15\times 10^{4}$ \\
$n_{\mathrm{H}}^{\mathrm{dust}}$ & $(\mathrm{cm}^{-3})$ & $1.35\times 10^{2}$ & $6.33\times 10^{2}$ & $2.96\times 10^{3}$ & $3.03\times 10^{2}$ & $8.10\times 10^{3}$ & $2.26\times 10^{3}$ & $1.03\times 10^{4}$ & $4.12\times 10^{4}$ & $5.60\times 10^{4}$ & $1.64\times 10^{4}$ & $2.48\times 10^{4}$ & $1.74\times 10^{4}$ & $2.22\times 10^{4}$ \\



==> tex/tab_value.tex <==
Molecule                                 & QNs                                                                                                  & Frequency                                & Noise    & Minimum  & Median   & Maximum  & Minimum  & Median   & Maximum  \\ 
                                         &                                                                                                      & (MHz)                                    & (K)      &          &          &          &          &          &          \\ 
\hline
$\ensuremath{\mathrm{^{12}CO}}$          & $\ensuremath{\mathrm{J=1 \rightarrow 0}}$                                                            &  115271.202                               & $  0.09$ & $ -0.39$ & $ 13.40$ & $ 57.11$ & $ -0.37$  & $  2.39$ & $  3.32$  \\ 
$\ensuremath{\mathrm{^{13}CO}}$          & $\ensuremath{\mathrm{J=1 \rightarrow 0}}$                                                            &  110201.3543                              & $  0.04$ & $ -0.19$ & $  1.38$ & $ 36.43$ & $ -0.19$  & $  0.97$ & $  3.03$  \\ 
$\ensuremath{\mathrm{CS}}$               & $\ensuremath{\mathrm{J=2 \rightarrow 1}}$                                                            &  97980.9533                               & $  0.06$ & $ -0.36$ & $  0.06$ & $ 15.53$ & $ -0.35$  & $  0.06$ & $  2.48$  \\ 
$\ensuremath{\mathrm{HCN}}$              & $\ensuremath{\mathrm{J=1 \rightarrow 0,\, F=2 \rightarrow 1}}$                                       &  88631.8475                               & $  0.10$ & $ -0.58$ & $  0.15$ & $ 10.32$ & $ -0.52$  & $  0.15$ & $  2.22$  \\ 
$\ensuremath{\mathrm{HCO^+}}$            & $\ensuremath{\mathrm{J=1 \rightarrow 0}}$                                                            &  89188.525                                & $  0.09$ & $ -0.45$ & $  0.26$ & $  8.07$ & $ -0.42$  & $  0.25$ & $  2.07$  \\ 
$\ensuremath{\mathrm{SO}}$               & $\ensuremath{\mathrm{J=3 \rightarrow 2,\, K=2 \rightarrow 1}}$                                       &  99299.87                                 & $  0.06$ & $ -0.43$ & $  0.04$ & $  6.46$ & $ -0.40$  & $  0.04$ & $  1.92$  \\ 
$\ensuremath{\mathrm{CN}}$               & $\ensuremath{\mathrm{N=1 \rightarrow 0,\, J=3/2 \rightarrow 1/2,\, F=5/2 \rightarrow 3/2 }}$         &  113490.9702                              & $  0.09$ & $ -0.58$ & $  0.10$ & $  6.33$ & $ -0.52$  & $  0.09$ & $  1.91$  \\ 
$\ensuremath{\mathrm{HNC}}$              & $\ensuremath{\mathrm{J=1 \rightarrow 0}}$                                                            &  90663.568                                & $  0.08$ & $ -0.49$ & $  0.07$ & $  6.01$ & $ -0.45$  & $  0.07$ & $  1.88$  \\ 
$\ensuremath{\mathrm{CCH}}$              & $\ensuremath{\mathrm{N=1 \rightarrow 0,\, J=3/2 \rightarrow 1/2,\, F=2 \rightarrow 1}}$              &  87316.898                                & $  0.12$ & $ -0.62$ & $  0.08$ & $  5.72$ & $ -0.55$  & $  0.08$ & $  1.85$  \\ 
$\ensuremath{\mathrm{C^{18}O}}$          & $\ensuremath{\mathrm{J=1 \rightarrow 0}}$                                                            &  109782.173                               & $  0.06$ & $ -0.30$ & $  0.06$ & $  5.55$ & $ -0.29$  & $  0.06$ & $  1.83$  \\ 
$\ensuremath{\mathrm{N_2H^+}}$           & $\ensuremath{\mathrm{J=1 \rightarrow 0,\, F1=2 \rightarrow 1,\, F=3 \rightarrow 2 }}$                &  93173.764                                & $  0.08$ & $ -0.44$ & $  0.00$ & $  4.53$ & $ -0.41$  & $  0.00$ & $  1.70$  \\ 
$\ensuremath{\mathrm{CH_3OH}}$           & $\ensuremath{\mathrm{J=2 \rightarrow 1,\, K=0 \rightarrow 0,\, (A+)}}$                               &  96741.375                                & $  0.06$ & $ -0.34$ & $  0.01$ & $  2.24$ & $ -0.32$  & $  0.01$ & $  1.26$  \\ 

